Robust and Parallel Bayesian Model Selection

Effective and accurate model selection is an important problem in modern data analysis. One of the major challenges is the computational burden required to handle large data sets that cannot be stored or processed on one machine. Another challenge one may encounter is the presence of outliers and contaminations that damage the inference quality. The parallel "divide and conquer" model selection strategy divides the observations of the full data set into roughly equal subsets and perform inference and model selection independently on each subset. After local subset inference, this method aggregates the posterior model probabilities or other model/variable selection criteria to obtain a final model by using the notion of geometric median. This approach leads to improved concentration in finding the "correct" model and model parameters and also is provably robust to outliers and data contamination.

==> proofs.tex <==
\section{SUPPLEMENTARY MATERIAL}
%\subsection*{Proofs}
%\subsubsection*{Proof of Theorem \ref{thm plain}}
%The proof is a modification of that for Theorem 2.1 in \cite{ghosal2000}. Take any $\epsilon>2\varepsilon_N$, we have, by Assumption \ref{assumption1},
%$$\log\mathcal D\left(\frac{\epsilon}{2},\mathcal P_{\mathcal S_N},d\right)\leq\log\mathcal D\left(\varepsilon_N,\mathcal P_{\mathcal S_N},d\right)\leq N\varepsilon_N^2$$
%Then, by Theorem 7.1 in \cite{ghosal2000}, there exists tests $\phi_N$ and a large enough constant $T$ (chosen later) such that
%\begin{equation}
%P_0^N\phi_N\leq e^{N\varepsilon_N^2}e^{-LNT^2\varepsilon_N^2}\frac{1}{1-e^{-LNT^2\varepsilon_N^2}}\label{test1}
%\end{equation}
%and
%\begin{equation}
%\sup_{\theta\in\mathcal S_N:d(P_\theta,P_0)>T\varepsilon_N}P_\theta^N(1-\phi_N)\leq e^{-LNT^2\varepsilon_N^2}\label{test2}
%\end{equation}
%for a universal constant $L>0$, any $N>0$, and $P_\theta^N$ denotes the probability measure on $(X,Y)$ under $(X_1,Y_1)\sim p_0(x)\times p_\theta(y|x)$.
%
%By \eqref{test1}, we have
%\begin{equation}
%P_0^NPr(\theta:\theta:d(P_\theta,P_0)>L\varepsilon_N^2|X,Y)\phi_N\leq P_0^N\phi_N\leq2e^{-LN\varepsilon_N^2}\label{interim5}
%\end{equation}
%as $N\to\infty$, if we choose $LT^2-1>L$. Now, since
%$$P_0\frac{p_\theta(Y_1|X_1)}{p_0(Y|X)}=\int\frac{p_\theta(y|x)}{p_0(y|x)}p_0(dy|x)p_0(dx)=\int p_\theta(dy|x)p_0(dx)=1$$
%by Fubini's theorem, we have
%$$P_0^N\int_{\mathcal S\setminus\mathcal S_N}\prod_{i=1}^N\frac{p_\theta(Y_i|X_i)}{p_0(Y_i|X_i)}Pr(\mathrm{d}\theta)\leq Pr(\mathcal S\setminus\mathcal S_N)$$
%Hence, by Fubini's theorem again,
%\begin{eqnarray}
%&&P_0^N\int_{\theta\in\mathcal S:d(P_\theta,P_0)>T\varepsilon_N}\prod_{i=1}^N\frac{p_\theta(Y_i|X_i)}{p_0(Y_i|X_i)}Pr(\mathrm{d}\theta)(1-\phi_N)\notag\\
%&\leq&\Pi(\mathcal S\setminus\mathcal S_N)+\int_{\theta\in\mathcal S_N:d(P_\theta,P_0)>T\varepsilon_N}P_\theta^N(1-\phi_N)Pr(\mathrm{d}\theta)\notag\\
%&\leq&\Pi(\mathcal S\setminus\mathcal S_N)+e^{-LNT^2\varepsilon_N^2}\text{\ \ by \eqref{test2}}\notag\\
%&\leq&2e^{-N\varepsilon_N^2(C+4)}\label{interim4}
%\end{eqnarray}
%if $KM^2\geq C+4$, by Assumption \ref{assumption2}.
%
%By Lemma \ref{lemma bound} (stated below) and Assumption \ref{assumption3}, with probability at least $1-1/(C^2N\varepsilon_N^2)$, we have
%\begin{equation}
%\int\prod_{i=1}^N\frac{p_\theta(Y_i|X_i)}{p_0(Y_i|X_i)}Pr(\mathrm{d}\theta)\geq e^{-2N\varepsilon_N^2}Pr(B_n)\geq e^{-N\varepsilon_N^2(2+C)}\label{interim3}
%\end{equation}
%where
%$$B_n=\left\{\theta:-P_0\log\frac{p_\theta(Y_1|X_1)}{p_0(Y_1|X_1)}\leq\varepsilon_N^2,\ P_0\left(\frac{p_\theta(Y_1|X_1)}{p_0(Y_1|X_1)}\right)^2\leq\varepsilon_N^2\right\}$$
%Let $A_N$ be the event that \eqref{interim3} holds. We have
%\begin{eqnarray*}
%&&P_0^NPr(\theta:d(P_\theta,P_0)>T\varepsilon_N|X,Y)(1-\phi_N)\mathbf 1_{A_N}\\
%&=&P_0^N\frac{\int_{\theta:d(P_\theta,P_0)>T\varepsilon_N}\prod_{i=1}^N\frac{p_\theta(Y_i|X_i)}{p_0(Y_i|X_i)}Pr(\mathrm{d}\theta)}{\int\prod_{i=1}^N\frac{p_\theta(Y_i|X_i)}{p_0(Y_i|X_i)}Pr(\mathrm{d}\theta)}(1-\phi_N)\mathbf 1_{A_N}\\
%&\leq&e^{N\varepsilon_N^2(2+C)}2e^{-N\varepsilon_N^2(C+4)}\text{\ \ by \eqref{interim4} and \eqref{interim3}}\\
%&=&2e^{-2N\varepsilon_N^2}\label{interim6}
%\end{eqnarray*}
%
%Therefore,
%\begin{eqnarray*}
%&&P_0^NPr(\theta:d(P_\theta,P_0)>T\varepsilon_N|X,Y)\\
%&=&P_0^NPr(\theta:d(P_\theta,P_0)>T\varepsilon_N|X,Y)\phi_N+P_0^NPr(\theta:d(P_\theta,P_0)>T\varepsilon_N|X,Y)(1-\phi_N)\mathbf 1_{A_N}{}\\
%&&{}+P_0^NPr(\theta:d(P_\theta,P_0)>T\varepsilon_N|X,Y)(1-\phi_N)(1-\mathbf 1_{A_N})\\
%&\leq&P_0^NPr(\theta:d(P_\theta,P_0)>T\varepsilon_N|X,Y)\phi_N+P_0^NPr(\theta:d(P_\theta,P_0)>T\varepsilon_N|X,Y)(1-\phi_N)\mathbf 1_{A_N}{}\\
%&&{}+P_0^N(A_N^c)\text{\ \ for sufficiently large $T$}\\
%&\leq&2e^{-LN\varepsilon_N^2}+2e^{-2N\varepsilon_N^2}+\frac{1}{C^2N\varepsilon_N^2}
%\end{eqnarray*}
%by \eqref{interim5}, \eqref{interim6} and the property of $A_N$. By Chebyshev's inequality, we have
%$$P_0^N\left(Pr(\theta:d(P_\theta,P_0)>T\varepsilon_N^2|X,Y)>\delta\right)\leq\frac{1}{C^2N\varepsilon_N^2\delta}+\frac{2e^{-LN\varepsilon_N^2}}{\delta}+\frac{2e^{-2N\varepsilon_N^2}}{\delta}$$
%which concludes the theorem.
%
%\begin{lemma}
%For any $\epsilon>0$ and probability distribution $\Pi$ defined on the set
%\begin{equation}
%\left\{\theta:-P_0\log\frac{p_\theta(Y|X)}{p_0(Y_1|X_1)}\leq\epsilon^2,\ P_0\left(\frac{p_\theta(Y|X)}{p_0(Y_1|X_1)}\right)^2\leq\epsilon^2\right\}\label{set}
%\end{equation}
%we have, for every $C>0$,
%\begin{equation}
%P_0^N\left(\int\prod_{i=1}^N\frac{p_\theta(Y_i|X_i)}{p_0(Y_i|X_i)}\Pi(\mathrm d\theta)\leq e^{-(1+C)N\epsilon^2}\right)\leq\frac{1}{C^2N\epsilon^2}\label{bound}
%\end{equation}\label{lemma bound}
%\end{lemma}
%
%The proof follows closely with Lemma 8.1 in \cite{ghosal2000}.
%
%\emph{Proof. }
%By Jensen's inequality, we have
%$$\log\int\prod_{i=1}^N\frac{p_\theta(Y_i|X_i)}{p_0(Y_i|X_i)}\Pi(\mathrm d\theta)\geq\int\sum_{i=1}^N\log\frac{p_\theta(Y_i|X_i)}{p_0(Y_i|X_i)}\Pi(\mathrm d\theta)$$
%Hence the left hand side of \eqref{bound} is bounded from above by
%\begin{equation}
%P_0^N\left(\mathcal G_N\int\log\frac{p_\theta(Y|X)}{p_0(Y_1|X_1)}\Pi(\mathrm d\theta)\leq-(1+C)\sqrt N\epsilon^2-\sqrt N P_0\int\log\frac{p_\theta(Y_1|X_1)}{p_0(Y_1|X_1)}\Pi(\mathrm d\theta)\right)\label{interim1}
%\end{equation}
%where $\mathcal G_N=\sqrt n(P_N-P_0)$ denotes the empirical process generated by $(X,Y)$, and $P_N$ here is the empirical distribution. Since $\Pi$ is defined on \eqref{set}, by Fubini's theorem, \eqref{interim1} is bounded further by
%\begin{equation}
%P_0^N\left(\mathcal G_N\int\log\frac{p_\theta(Y|X)}{p_0(Y|X)}\Pi(\mathrm d\theta)\leq-C\sqrt N\epsilon^2\right)\label{interim2}
%\end{equation}
%By Chebyshev's inequality, \eqref{interim2} is bounded by
%$$\frac{Var_0\left(\int\log\frac{p_\theta(Y_1|X_1)}{p_0(Y_1|X_1)}\Pi(\mathrm d\theta)\right)}{C^2N\epsilon^4}$$
%where $Var_0$ denotes the variance under $P_0$, which is in turn bounded by
%$$\frac{P_0\left(\int\log\frac{p_\theta(Y_1|X_1)}{p_0(Y_1|X_1)}\Pi(\mathrm d\theta)\right)^2}{C^2N\epsilon^4}\leq\frac{\int P_0\left(\log\frac{p_\theta(Y_1|X_1)}{p_0(Y_1|X_1)}\right)^2\Pi(\mathrm d\theta)}{C^2N\epsilon^4}$$
%by Jensen's inequality and Fubini's theorem again. The last expression is bounded by $1/(C^2N\epsilon^2)$ since $\Pi$ is defined on \eqref{set}.
%
%
%\subsubsection*{Proof of Theorem \ref{thm model selection}}
%\emph{Proof of \ref{plain}.} Consider $N\to\infty$ and fix a $T>0$. We have
%\begin{eqnarray}
%&&Pr(\theta:d(P_\theta,P_0)\leq T\varepsilon_N^2|X,Y)\notag\\
%&=&E_{Pr}\left[Pr(\theta:d(P_\theta,P_0)\leq T\varepsilon_N^2|M_k,X,Y)|X,Y\right]{}\\
%&&{}\text{\ \ where $E_{Pr}[\cdot|X,Y]$ denotes the posterior expectation}{}\notag\\
%&&{}\text{\ \ and $Pr(\cdot|M_k,X,Y)$ denotes the posterior distribution given model $M_k$}\notag\\
%&=&Pr(M_1|X,Y)Pr(\theta:d(P_\theta,P_0)\leq T\varepsilon_N^2|M_1,X,Y)\label{interim14}
%\end{eqnarray}
%by the condition that $d(P_\theta,P_0)>M\varepsilon_N^2$ for any $\theta\in\mathcal S_{-1}$ eventually. Hence
%\begin{equation}
%Pr(\theta:d(P_\theta,P_0)\leq M\varepsilon_N^2|X,Y)\geq1-\delta\label{interim7}
%\end{equation}
%implies
%\begin{equation}
%Pr(M_1|X,Y)\geq1-\delta\label{interim8}
%\end{equation}
%The result then follows from Theorem \ref{thm plain}, which implies that \eqref{interim7} occurs with probability at least
%$$1-\left(\frac{1}{C^2N\varepsilon_N^2\delta}+\frac{2e^{-LN\varepsilon_N^2}}{\delta}+\frac{2e^{-2N\varepsilon_N^2}}{\delta}\right)$$
%\begin{equation}
%P_0^N\left(Pr(M_1|X,Y)<1-\delta\right)\leq\frac{1}{C^2N\varepsilon_N^2\delta}+\frac{2e^{-LN\varepsilon_N^2}}{\delta}+\frac{2e^{-2N\varepsilon_N^2}}{\delta}\label{interim9}
%\end{equation}
%
%\emph{Proof of \ref{Euclidean}.}
%Note that \eqref{interim8} implies
%\begin{equation}
%d_E(Pr(M_k|X,Y),\mathbf e_1)=\sqrt{(1-Pr(M_1|X,Y))^2+\sum_{k\neq1}Pr(M_k|X,Y)^2}\leq\sqrt2\delta\label{interim10}
%\end{equation}
%since $(1-Pr(M_1|X,Y))^2\leq\delta^2$ and
%$(\delta,0,\ldots,0)$ is an optimizer of the optimization
%$$\max\sum_{i=2}^Kx_i^2\text{\ \ subject to\ \ }\sum_{i=2}^Kx_i\leq\delta$$
%Hence \eqref{interim9} and \eqref{interim10} together imply
%$$P_0^N\left(d_E(Pr(M_k|X,Y),\mathbf e_1)\geq\sqrt2\delta\right)\leq\frac{1}{C^2N\varepsilon_N^2\delta}+\frac{2e^{-LN\varepsilon_N^2}}{\delta}+\frac{2e^{-2N\varepsilon_N^2}}{\delta}$$
%By redefining $\tilde\delta=\sqrt2\delta$, we get \eqref{Euclidean bound}.
%
%\emph{Proof of \ref{Hellinger}.}
%Note that \eqref{interim8} implies
%\begin{align}
%d_H(Pr(M_k|X,Y),\mathbf e_1)&=\sqrt{\frac{1}{2}\left((\sqrt{1-Pr(M_1|X,Y)})^2+\sum_{k\neq1}Pr(M_k|X,Y)\right)}\notag\\
%&\leq\sqrt{\frac{1}{2}\left((1-\sqrt{1-\delta})^2+\delta\right)}\label{interim11}
%\end{align}
%since $x_i=\delta/(k-1)$ for all $i\neq0$ gives the optimizer of the optimization
%$$\max\sum_{i\neq0}\sqrt{x_i}\text{\ \ subject to\ \ }\sum_{i\neq0}x_i\leq\delta$$
%Hence \eqref{interim9} and \eqref{interim11} together imply
%\begin{equation}
%P_0^N\left(d_H(Pr(M_k|X,Y),\mathbf e_1)>\sqrt{\frac{1}{2}\left((1-\sqrt{1-\delta})^2+\delta\right)}\right)\leq\frac{1}{C^2N\varepsilon_N^2\delta}+\frac{2e^{-LN\varepsilon_N^2}}{\delta}+\frac{2e^{-2N\varepsilon_N^2}}{\delta}\label{interim12}
%\end{equation}
%Note that $(1-\sqrt{1-\delta})^2$ is a convex function in $\delta$ for $0<\delta<1$ and is equal to 0 at $\delta=0$. Thus $(1-\sqrt{1-\delta})^2\leq(\sqrt 2-1)^2\delta$ for $0<\delta<1/2$, where $(\sqrt 2-1)^2$ is the slope of the line between $(0,0)$ and $(1/2,(1-\sqrt{1-1/2})^2$. Hence, for $0<\delta<1/2$, we have
%$$\sqrt{\frac{1}{2}\left((1-\sqrt{1-\delta})^2+\delta\right)}\leq\sqrt{((\sqrt 2-1)^2+1)\frac{\delta}{2}}$$
%Combining with \eqref{interim12}, we have
%$$P_0^N\left(d_H(Pr(M_k|X,Y),\mathbf e_1)>\sqrt{((\sqrt 2-1)^2+1)\frac{\delta}{2}}\right)\leq\frac{1}{C^2N\varepsilon_N^2\delta}+\frac{2e^{-LN\varepsilon_N^2}}{\delta}+\frac{2e^{-2N\varepsilon_N^2}}{\delta}$$
%By redefining $\tilde\delta=\sqrt{((\sqrt 2-1)^2+1)\delta/2}$, we get \eqref{Hellinger bound}.
%
%\begin{remark}
%Note that the concentration bound for Hellinger distance \eqref{Hellinger bound} is inferior to that for Euclidean distance \eqref{Euclidean bound} for small $\delta$ since $\delta^2$ instead of $\delta$ shows up in the RHS of \eqref{Hellinger bound}. This is because in our proof, the function $\sqrt{(1-\sqrt{1-\delta})^2+\delta}$ that appears in \eqref{interim12} has derivative $1/(2\sqrt{(1-\delta)((1-\sqrt{1-\delta})^2+\delta)})$ which is $\infty$ at $\delta=0$, and thus no linearization is available when $\delta$ is close to 0. In this sense the bound in \eqref{Hellinger bound} cannot be improved.
%\end{remark}
%
%\subsubsection*{Proof of Theorem \ref{thm main} and \ref{thm extension}}
%The proofs of both theorems rely on a key theorem on geometric median in \cite{minsker2015geometric}, restated below:
%\begin{thm}
%Consider a Hilbert space $(\mathbb H,\langle\cdot,\cdot\rangle)$ and $\xi_0\in\mathbb H$. Let $\hat\xi_1,\ldots,\hat\xi_R\in\mathbb H$ be a collection of independent random $\mathbb H$-valued elements. Let  $\alpha,q,\nu$ be constants such that $0<q<\alpha<1/2$ and $0\leq\nu<(\alpha-q)/(1-q)$. Suppose that there exists $\epsilon>0$ such that for all $j$, where $1\leq j\leq\lfloor(1-\nu)R\rfloor+1$,
%$$P(\|\hat\xi_j-\xi_0\|>\epsilon)\leq q$$
%Let $\hat\xi_*=\text{med}_g(\hat\xi_1,\ldots,\hat\xi_R)$ be the geometric median of $\{\hat\xi_1,\ldots,\hat\xi_R\}$. Then
%$$P(\|\hat\xi_*-\xi_0\|>C_\alpha\epsilon)\leq\left(e^{(1-\nu)\psi(\frac{\alpha-\nu}{1-\nu},q)}\right)^{-R}$$
%where $C_\alpha=(1-\alpha)\sqrt{1/(1-2\alpha)}$, and
%$$\psi(\alpha,q)=(1-\alpha)\log\frac{1-\alpha}{1-q}+\alpha\log\frac{\alpha}{q}$$\label{thm geometric median}
%\end{thm}
%
%We focus on Theorem \ref{thm main}. The proof for Theorem \ref{thm extension} is a straightforward modification in light of Theorem \ref{thm geometric median}.
%
%\emph{Proof of \ref{geometric median Euclidean}.}
%Immediate by noting that
%$$P_0^s\left(d(Pr(M_k|X_{(j)},Y_{(j)}),\mathbf e_1)>\delta\right)\leq q$$
%for all $j=1,\ldots,R$, and applying Theorem \ref{thm geometric median}.
%
%\emph{Proof of \ref{geometric median plain}.}
%Note that
%\begin{equation}
%d_E(Pr_*(M_k|X,Y),\mathbf e_1)\geq(1-Pr_*(M_1|X,Y))\sqrt{\frac{K}{K-1}}\label{interim13}
%\end{equation}
%To see this, let $a=Pr_*(M_1|X,Y)$. We have $d_E(Pr_*(M_k|X,Y),\mathbf e_1)=\sqrt{(1-a)^2+\sum_{i=2}^Kx_i^2}$ where $x_i$'s satisfy $\sum_{i=2}^Kx_i=1-a$. Since $(1-a)/(K-1)$ is the optimizer of the optimization
%$$\min\sum_{i=2}^Kx_i^2\text{\ \ subject to\ \ }\sum_{i=2}^Kx_i=1-a$$
%we get $\sqrt{(1-a)^2+\sum_{i=2}^Kx_i^2}\geq(1-a)\sqrt{K/(K-1)}$.
%
%Hence \eqref{geometric median Euclidean bound} and \eqref{interim13} together give
%$$P_0^N\left(Pr_*(M_1|X,Y)<1-C_\alpha\delta\sqrt{\frac{K-1}{K}}\right)\leq\left(e^{(1-\nu)\psi(\frac{\alpha-\nu}{1-\nu},q)}\right)^{-R}$$
%
%\emph{Proof of \ref{geometric median joint}.}
%By using the same thread of argument as in \eqref{interim14}, we have
%$$Pr(\theta:d(P_\theta,P_0)\leq T\varepsilon_N^2|X,Y)\geq1-\delta$$
%implies
%$$Pr(\theta:d(P_\theta,P_0)\leq T\varepsilon_N^2|M_1,X,Y)\geq1-\delta$$
%for any $0<\delta<1$. Hence \eqref{main plain} implies that
%$$P_0^N\left(Pr(\theta:d(P_\theta,P_0)>T\varepsilon_N^2|M_1,X,Y)>\delta\right)\leq\frac{1}{C^2N\varepsilon_N^2\delta}+\frac{2e^{-LN\varepsilon_N^2}}{\delta}+\frac{2e^{-2N\varepsilon_N^2}}{\delta}$$
%and by the additional assumption we have
%$$P_0^N\left(Pr(\theta:\tilde Cd_{\mathcal F}(P_\theta,P_0)^\gamma>T\varepsilon_N^2|M_1,X,Y)>\delta\right)\leq\frac{1}{C^2N\varepsilon_N^2\delta}+\frac{2e^{-LN\varepsilon_N^2}}{\delta}+\frac{2e^{-2N\varepsilon_N^2}}{\delta}$$
%Applying a union bound, we get
%\begin{eqnarray*}
%&&P_0^N\Bigg(Pr_*(M_1|X,Y)>1-C_\alpha\delta\sqrt{\frac{K-1}{K}},\\
%&&{}\ Pr_*\left(\theta:d_{\mathcal F}(P_\theta,P_0)\leq\left(\frac{T}{\tilde C}\varepsilon_N^2\right)^{1/\gamma}\Bigg|M_1,X,Y\right)\geq1-\delta\Bigg)\\
%&\geq&1-2\left(e^{(1-\nu)\psi(\frac{\alpha-\nu}{1-\nu},q)}\right)^{-R}
%\end{eqnarray*}
%
%
%\subsection*{Gibbs Sampler for Parallel MCMC for Spike and Slab Prior}
%For posterior inference in the spike and slab model, let $\Delta = \text{diag}\left\{ J_1\tau_{1}^{2}, \ldots , J_D\tau_{D}^{2} \right\}$,  we can perform Gibbs sampling by drawing from the following posteriors:
%\begin{align}
%Pr(\beta_{SS} | - ) &\sim N(\mu_{\beta_{SS}}, \Sigma_{\beta_{SS}}),\\
% \Sigma_{\beta_{SS}} &= \left( \Delta^{-1} + \frac{P}{N\sigma^2} X^TX \right)^{-1},\; \mu_{\beta_{SS}} = \Sigma_{\beta_{SS}} \left( \frac{P}{N\sigma^2} X^TY \right),\\
%Pr\left( \sigma^{-2}_{SS} | - \right) &\sim \text{Gamma}\left( a + \frac{N}{2}, b + \frac{P}{2N}\left(Y - X\beta \right)^T \left(Y - X\beta \right) \right)\\
%\begin{split}
%Pr\left( J_d | - \right) &\propto w_{d1} \delta_{J_d}(\nu_0) + w_{d2}\delta_{J_d}(1)\\
%w_{d1} &= (1-w)\nu_0^{-1/2}\exp\left\{ -\frac{\beta_{d}^2}{2\nu_0\tau^{2}_{d}} \right\}\\
%w_{d2} &= w \exp\left\{ -\frac{\beta^{2}_{d}}{2\tau^{2}_{d}} \right\}
%\end{split}\\
%Pr\left( \tau^{-2}_{d} | - \right) &\sim \text{Gamma}\left( a_{\tau} + \frac{1}{2}, b_{\tau} + \frac{\beta^{2}_{d}}{2J_{d}} \right)\\
%Pr(w | -) &\sim \text{Beta}\left( 1+ \left| \left\{ d : J_d = 1 \right\} \right| , 1+ \left| \left\{ d : J_d = \nu_0 \right\} \right| \right)
%\end{align}

%\subsubsection*{Additional Results and Plots From Simulation Studies}
%
%\begin{figure}[hbtp]
%	\centering
%	\includegraphics[width=0.9\linewidth]{big_contam_bma_med_10.png}
%	\caption{Contamination test}
%\end{figure}
%
%\begin{figure}[hbtp]
%	\centering
%	\includegraphics[width=0.9\linewidth]{big_contam_aic_bic_10.png}
%	\caption{Contamination test}
%\end{figure}
%
%
%\begin{figure}[hbtp]
%	\centering
%	\includegraphics[width=0.9\linewidth]{big_contamination_ss_10.png}
%	\caption{Contamination test.}
%\end{figure}
%
%\begin{figure}[hbtp]
%	\centering
%	\includegraphics[width=0.9\linewidth]{big_cover_aic_bic.png}
%	\caption{Coverage test.}
%\end{figure}
%
%\begin{figure}[hbtp]
%	\centering
%	\includegraphics[width=0.9\linewidth]{big_cover_med_bma.png}
%	\caption{Coverage test.}
%\end{figure}
%
%\begin{figure}[hbtp]
%	\centering
%	\includegraphics[width=0.9\linewidth]{big_coverage_ss.png}
%	\caption{Coverage test.}
%	
%\end{figure}
%
%
%\begin{figure}[hbtp]
%	\centering
%	\includegraphics[width=0.9\linewidth]{big_mag_aic_bic.png}
%	\caption{Magnitude test.}
%	
%\end{figure}
%
%\begin{figure}[hbtp]
%	\centering
%	\includegraphics[width=0.9\linewidth]{big_mag_bma_med.png}
%	\caption{Magnitude test.}
%\end{figure}
%
%\begin{figure}[hbtp]
%	\centering
%	\includegraphics[width=0.9\linewidth]{big_magnitude_ss.png}
%	\caption{Magnitude test.}
%\end{figure}

%The diabetes data consists of a $442 \times 10$ dimension design matrix scaled with unit norm and zero mean and a single response vector. We held out $45$ observations for test evaluation and plotted the posterior $95\%$ credible intervals for the predictive values centered at zero after subtracting the true predictive value. We can see that, after dividing the data across 5 subsets, we can attain a tighter credible interval over the true value for each model selection technique.
%
%\begin{figure}[hbtp]
%\centering
%\includegraphics[width=0.7\linewidth]{diabetes_ss.png}
%\caption{Diabetes test data.}
%\end{figure}
%
%\begin{figure}[hbtp]
%\centering
%\includegraphics[width=0.7\linewidth]{figs/diabetes_coverage_aic_bic.png}
%\caption{Diabetes test data.}
%\end{figure}
%
%\begin{figure}[hbtp]
%\centering
%\includegraphics[width=0.7\linewidth]{figs/diabetes_coverage_med_bma.png}
%\caption{Diabetes test data.}
%\end{figure}
%
%For the regression coverage tests, the true model has 3 true predictors. The first 3 regression coefficients have values $-1.2, 4.3, 2.2$ and the rest are zero.
%
%\begin{figure}[hbtp]
%\centering
%\includegraphics[width=0.7\linewidth]{figs/regression_coverage_5_model_estimate_combine.png}
%\caption{Comparison of estimate and model combination for 5 subsets}
%\end{figure}

%\begin{figure}[hbtp]
%\centering
%\includegraphics[width=0.7\linewidth]{figs/regression_coverage.png}
%\caption{Regression coverage of estimate combination betwwen 1 and 5 subsets.}
%\end{figure}
